Robustness of DC Power Networks under Weight Control

We study, possibly distributed, robust weight control policies for DC power networks that change link susceptances, or weights in response to balanced disturbances to the supply-demand vector. The margin of robustness for a given control policy is defined as the radius of the largest $l_1$ ball in the space of balanced disturbances under which the link flows can be asymptotically contained within their specified limits. For centralized control policies, the control design as well as margin of robustness are obtained from solution to an non-convex weight control problem. We establish relationship between feasible sets for DC power flow and associated network flow, which is used to establish an upper bound on the margin of robustness in terms of the min cut capacity. This bound is proven to be tight if the network is tree-like, or if the lower bound of the operation range of weight control is zero. An explicit expression for the flow-weight Jacobian is derived and is used to devise a projected sub-gradient algorithm to solve the relaxed weight control problem. An exact multi-level programming approach to solve the weight control problem for reducible networks, based on recursive application of equivalent bilevel formulation for relevant class of non-convex network optimization problems, is also proposed. The lower level problem in each recursion corresponds to replacing a sub-network by a (virtual) link with equivalent weight and capacities. The equivalent capacity function for tree-reducible networks is shown to possess a strong quasi-concavity property, facilitating easy solution to the weight control problem. Robustness analysis for natural decentralized control policies that decrease weights on overloaded links, and increase weights on underloaded links with increasing flows is provided for parallel networks. Illustrative simulation results for a benchmark IEEE network are included.

==> multigraph.tex <==
\subsection{Extension to Multigraphs}
\label{sec:multigraph}
%A \emph{multigraph} is a graph which is permitted to have  multiple edges, \ie
%parallel edges incident to the same nodes. Eq. (\ref{eq:sol}) encapsulates the
%physical law of the DC power flow model (\ref{model}) and provides the flow
%solution for a given load upon a given network. However, since the Laplacian
%matrice are usually employed for simple graphs, we confine the applicability of
%Eq. (\ref{eq:sol}) within simple graphs. In this subsection, we show that the
%same equation holds for multigraph. Furthermoer, there is some interesting
%relationship between weight decrease and failure of links when multigraph is
%considered. 

%\ksmargin{an illustrative figure here would be helpful}
%Eq. \eqref{eq:sol} is applicable only to simple graphs, i.e., graphs where there exists at most one link between a given pair of nodes. In this section, we investigate its applicability to \emph{multigraphs}. A multigraph is a graph which allows multiple links between a given pair of nodes. Eq. \eqref{eq:sol} is extended to multigraphs via an equivalent \emph{reduced} simple graph. Given a multigraph $\mc G=(\mc V, \mc E)$ with weights $w$, its equivalent reduced graph 

% The distinction between a multigraph and a simple graph is that the node-link
% incidence matrix \( A \) of a multigraph 
%contains identical columns. Since a column \( a_{i} \) of the node-link
%incidence mattrix \( A \) denotes
%the link \( i \), multi-edges, say link \( i \) and \( j \) which connects the
%same nodes have the same corresponding column, \ie \( a_{i} = a_{j} \). To make the difference
%clear, we denote the node-link incidence matrix of a multigraph of \( n \)
%nodes and \( m \) links using \( A_{M}\in \real^{n\times m_{1}} \).
%Correspondingly, let \( w_{M}\in \real^{m_{1}\times m_{1}} \) denote the weight
%matrix. \( L_{M} = A_{M}w_{M}\trans{A_{M}} \) can be seen as the
%Laplacian matrix of the multigraph. 
%
%Let \( A \in \real^{n\times m} \) be the
% matrix after removing the replicate columns from \( A_{M}\). Then \( A \) is
% the node-link incidence matrix of a simple graph after replacing all the
% multiple edges in the original multigraph with single links. The node sets in
% the two graph are the same, but the link sets are different. In particular, \(
% m_{1} = \sum_{i=1}^{m} |\mathcal{M}_{i}|  \), where \( \mathcal{M}_{i} \) is
% the set of links in the multigraph which has the same incident nodes as link \(
% i \) in the simple graph. Let \( w\in \real^{m\times m} \) with  \( w_{i} =
% \sum_{j\in \mathcal{M}_{i}} w_{j} \) be the weight matrix of the simple
% graph. We call the simple graph the \emph{base graph} of the multigraph
% graph. And they have the following relationship. 

%It is one-to-one correspondance between a simple graph and Laplacian
%matrix. However, Lemma \ref{lem:base-graph-laplacian} shows that multiple
%graphs can have the same Laplacian matrix when multiple graphs are
%considered. In particular, a simple graph is the base graph of infinitely many
%multigraphs and all these multigraphs have the same Laplacian matrix. 

\kscomment{Lemma~\ref{lem:base-graph-laplacian} implies that Lemma~\ref{lemma:flow-solution} can be extended for a multigraph $\mc G$ satisfying Assumption~\ref{ass:connectivity}, and weight matrix $w$ as follows. For every $p$ satisfying Assumption~\ref{ass:balanced}, there exists a unique $f \in \RR^{\mc E}$ satisfying \eqref{model}, and is given by:
\begin{equation}
\label{eq:flow-solution-multigraph}
f = w \trans{A} L_{eq}^{\dagger} p
\end{equation}
}

%Since Eq. (\ref{model}) describes the relationship of the quantities dictated by
%the physical law of DC power networks, it remains to be true for multigraphs.
%Due to Lemma \ref{lem:base-graph-laplacian}, the properties that a Laplacian
%matrix possesses remains to be true for Laplacian matrices of multigraphs.
%Hence, unique solution of flow to (\ref{model}) exists for multigraph, and is
%given by 
%\begin{equation}
%\label{eq:flow-solution-multigraph}
%f_{M} = w_{M} \trans{A_{M}} L^{\dagger} p
%\end{equation}
%where \( L \) is the Laplacian matrix of the base graph of the multigraph. 
\ksmargin{need to verify this claim}
\kscomment{
It is easy to verify that Lemma \ref{lemma:Jacobian} also extends to 
multigraphs, thereby also allowing to extend the projected gradient descent algorithm from Section~\ref{subsec:gradient-descent} to multigraphs. 
}
%Also, in the following of this paper, we use
%Eq. (\ref{eq:sol}) as the flow solution to both simple graphs and multigraphs
%without mentioning the difference. 

\ksmargin{this paragraph looks redundant}
\kscomment{
Furthermore, the folow solution (\ref{eq:flow-solution-multigraph}) of a
multiple can also be obtained from the flow solution of its base graph. 
Notice \( w_{i} = \sum_{j\in \mathcal{M}_{i}} w_{j}\), link \( i \) in base
graph can be seen as an equivalence of the link set \( \mathcal{M}_{i} \) of the
original multigraph. We can first solve the flow of the base graph as  \( f =
w\trans{A}L^{\dagger} p \). \( f_{i} \) is the flow on link \( i \) of the base
graph, and also the resultant flow into link set \( \mathcal{M}_{i} \) of the
multigraph. And the flow on link \( j \in \mathcal{M}_{i} \) is obtained as  \(
f_{j} = f_{i} w_{j}/w_{i} \) by solving locally the parallel connected network
structure whose link set is \( \mathcal{M}_{i} \). Let \( Q = \diag\{q_{1},
q_{2}, \ldots, q_{m}\}\in \real^{m_{1}\times m} \) with \( q_{i} =
w_{\mathcal{M}_{i}}/w_{i}\). Then the flow solution of the multigraph can be
written as follows. 
\begin{equation}
\label{eq:flow-solution-multigraph-2}
  f_{M} = Q f = Q w \trans{A} L^{\dagger}p
\end{equation}
It is easy to check that Eq. (\ref{eq:flow-solution-multigraph}) and
(\ref{eq:flow-solution-multigraph-2}) are equivalent. 
}

%Now we've seen that there exists an equivalence relationsip between a multigraph
%and its base graph. (By equivalence, we mean roughly the same flow solution. It
%is possible to define the equivalence relationship formally.) To solve the flow
%of a network, it is possible to solve the 
%flow solution of the equivalent network first, and then use the solution to
%obtain the flow solution of the original network by solving some local network
%structures. \ksmargin{reference ?}
%\kscomment{This equivalent transformation of network topology is known in classical circuit
%theory.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../acc16"
%%% End:

